MOEA/D with Random Partial Update Strategy

Recent studies on resource allocation suggest that some subproblems are more important than others in the context of the MOEA/D, and that focusing on the most relevant ones can consistently improve the performance of that algorithm. These studies share the common characteristic of updating only a fraction of the population at any given iteration of the algorithm. In this work we investigate a new, simpler partial update strategy, in which a random subset of solutions is selected at every iteration. The performance of the MOEA/D using this new resource allocation approach is compared experimentally against that of the standard MOEA/D-DE and the MOEA/D with relative improvement-based resource allocation. The results indicate that using the MOEA/D with this new partial update strategy results in improved HV and IGD values, and a much higher proportion of non-dominated solutions, particularly as the number of updated solutions at every iteration is reduced.

==> files/5_steadystate.tex <==
\section{MOEA/D-PS and Steady State Evolutionary Algorithm}

In this Section we compare MOEA/D-PS with steady state MOEA/Ds, since it is in our understanding that MOEA/D-PS share some characteristics with steady state~\footnote{"The name steady state is somewhat unfortunate, since not all EAs display steady state behaviour~\cite{whitley2006alternative}.} MOEA/Ds.

We use the definition of steady-state EA from B{\"a}ck~\cite{back2018evolutionary}. It follows as; "Steady-state EAs are systems in which usually only one or two offspring are produced in every generation. "Generational systems are so named because the entire population is replaced every generation by the offspring population: the lifetime of each individual in the population is only one generation. This is the same as the non-overlapping population systems, while the steady-state EA is an overlapping population system". This definition is reinforced by the works of Durillo et. al~\cite{durillo2009effect}, Li et. al~\cite{li2014efficient}, Yagoubi et. al~\cite{yagoubi2012asynchronous} and others.

Considering only the (non-)overlapping population criterion, steady-state EAs might be seen as:
\begin{itemize}
    % \item algorithms that generate only few solutions at every iteration;
    \item algorithms that update only few solutions at every iteration.
    \item algorithms that have overlapping solutions - solutions generated in many different iterations.
\end{itemize}

\subsection{Advantages of steady EAs} Li et. al~\cite{li2014efficient} suggest that steady-state EA have better chances for creating promising solutions, are easier to be implemented for parallel environments and are more feasible for theoretical analysis than generational EAs. In addition to that,  Yagoubi et. al~\cite{yagoubi2012asynchronous} justify that steady-state EAs might be more suitable to some problems than generational EAs by speeding-up the search procedure by inserting back in the set of solutions each generated solutions  as soon as it has been evaluated. Furthermore, Chafekar et. al~\cite{chafekar2003constrained} recommend steady-state EAs for problems with complex search space, with many constraints and with small feasible non-negligible amount of time.

\subsection{MOEA/D and Steady State EAs}

It is possible to understand that MOEA/D already shows some steady state characteristics, since this algorithm can have some solutions from many different iterations. That is because it is possible that the set of solutions on MOEA/D change only partially from one iteration to the next, specially on the final iterations of the search when it becomes harder to generate new, better solutions. In this scenario, we understand that MOEA/D-PS intensifies this behavior of MOEA/D, hence only few solutions can be updated at every iteration, staggering even further the set of solutions and making it easier to have solutions generated in many different iterations.

We highlight the following studies on steady state MOEA/Ds. Li et.a al~\cite{li2017new} proposes MOEA/D-II, in which only one solution is selected for local search in each iteration. Jiang et al.~\cite{jiang2016steady} proposes a new algorithm, SGEA that among other things, use a steady-state change detection mechanism. They compare the SGEA with a MOEA/D using this new update strategy, updating a maximum 10\% of the set of population.

\subsection{MOEA/D with priority functions and Steady State EAs}~\label{steadystate_ea}

We understand that MOEA/D with any Priority Function display some steady state characteristics, such generating and updating only a a small fraction of the total set of population given the Partial Update Strategy as well as having in the set of solution overlapping solutions (solutions from many different iterations).  


\subsection{MOEA/D-PS and Steady State Evolutionary Algorithm}

The Partial Update Strategy makes MOEA/D only update only some solutions. On our experiments, the best proportion of the set of solutions to be update was around 10\% of the population. Although in this study we limit the proportion of update solutions to around 10\%, MOEA/D-PS could use even smaller values of its control parameter, updating even less solutions. Therefore, from the point of view of solutions updated, MOEA/D-PS already displays some steady state behavior, as well as a similar behaviors with other variants from the literature~\cite{jiang2016steady}. 









==> files/hv_medians.tex <==
\begin{table*}[!t]
	\centering
	\normalsize
	\caption[HV medians and standard deviations.]{HV medians and standard deviations (in parenthesis) for every problem and technique. The best point value for each problem is indicated in boldface.}
	\label{table_hv_threshold}
	\begin{tabular}{lllllll}
	\hline
		\rowcolor[gray]{.7} \multicolumn{1}{|l|}{\textbf{HV}}         & \multicolumn{1}{l|}{10\%} & \multicolumn{1}{l|}{20\%} & \multicolumn{1}{l|}{40\%} & \multicolumn{1}{l|}{60\%} & \multicolumn{1}{l|}{80\%} & \multicolumn{1}{l|}{100\%} \\ \hline \hline  \hline
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF1}  
		& \multicolumn{1}{l}{\textbf{0.850 (0.023)}} 
		& \multicolumn{1}{l}{\textbf{0.850 (0.023)}} 
		& \multicolumn{1}{l}{ 0.823 (0.023)} 
		& 0.777 (0.023)            
		&\multicolumn{1}{l} {0.764 (0.026)} &\multicolumn{1}{l} {0.738 (0.025)}\\ 
		
		\multicolumn{1}{l}{UF2}  
		& \multicolumn{1}{l}{ 0.788 (0.025)} 
		& \multicolumn{1}{l}{0.794 (0.021)}
		& \multicolumn{1}{l}{ 0.792 (0.018)} 
		& 0.781 (0.017)            
		&\multicolumn{1}{l} {0.778 (0.023)} &\multicolumn{1}{l} {0.760 (0.018)}\\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF3}  
		& \multicolumn{1}{l}{\textbf{0.561 (0.058)}} 
		& \multicolumn{1}{l}{0.557 (0.057)} 
		& \multicolumn{1}{l}{ 0.545 (0.035)} 
		& 0.536 (0.032)            
		&\multicolumn{1}{l} {0.526 (0.027)} &\multicolumn{1}{l} {0.516 (0.019)}\\ 
		
		\multicolumn{1}{l}{UF4}  
		& \multicolumn{1}{l}{ 0.372 (0.004)} 
		& \multicolumn{1}{l}{\textbf{0.373 (0.004)}} 
		& \multicolumn{1}{l}{ 0.370 (0.003)} 
		& 0.368 (0.004)            
		&\multicolumn{1}{l} {0.368 (0.004)} &\multicolumn{1}{l} {0.366 (0.004)} \\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF5}  
		& \multicolumn{1}{l}{0.717 (0.031)}
		& \multicolumn{1}{l}{\textbf{0.727 (0.029)}} 
		& \multicolumn{1}{l}{0.689 (0.027)} 
		& 0.660 (0.027)            
		&\multicolumn{1}{l} {0.634 (0.023)} &\multicolumn{1}{l} {0.570 (0.023)} \\ 
		
		\multicolumn{1}{l}{UF6}  
		& \multicolumn{1}{l}{\textbf{0.816 (0.030)}} 
		& \multicolumn{1}{l}{0.813 (0.030)} 
		& \multicolumn{1}{l}{ 0.772 (0.033)} 
		& 0.749 (0.029)            
		&\multicolumn{1}{l} {0.724 (0.038)} &\multicolumn{1}{l} {0.687 (0.034)}\\
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF7}  
		& \multicolumn{1}{l}{\textbf{0.840 (0.027)}}
		& \multicolumn{1}{l}{0.816 (0.023)} 
		& \multicolumn{1}{l}{0.777 (0.026)} 
		& 0.753 (0.024)            
		&\multicolumn{1}{l} {0.732 (0.030)} &\multicolumn{1}{l} {0.706 (0.023)} \\
		
		\multicolumn{1}{l}{UF8}  
		& \multicolumn{1}{l}{\textbf{0.854 (0.008)}}
		& \multicolumn{1}{l}{0.854 (0.009)} 
		& \multicolumn{1}{l}{0.839 (0.009)} 
		& 0.829 (0.010)            
		&\multicolumn{1}{l} {0.821 (0.011)} &\multicolumn{1}{l} {0.806 (0.014)}\\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF9}  
		& \multicolumn{1}{l}{\textbf{0.767 (0.032)}}
		& \multicolumn{1}{l}{0.761 (0.025)} 
		& \multicolumn{1}{l}{0.745 (0.022)} 
		& 0.747 (0.020)            
		&\multicolumn{1}{l} {0.738 (0.023)} &\multicolumn{1}{l} {0.727 (0.025)} \\ 
		
		
		
		\multicolumn{1}{l}{UF10}              & \multicolumn{1}{l}{\textbf{0.807 (0.057)}}
    		& \multicolumn{1}{l}{0.785 (0.036)} 
    		& \multicolumn{1}{l}{0.735 (0.035)}
    		& 0.725 (0.028)             
    		&\multicolumn{1}{l} {0.690 (0.033)} &\multicolumn{1}{l} {0.671 (0.028)}  \\ 
		\hline \hline \hline
		
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ1}  
		& \multicolumn{1}{l}{\textbf{0.999 (0.001)}} 
		& \multicolumn{1}{l}{0.999 (0.002)} 
		& \multicolumn{1}{l}{0.999 (0.002)} 
		& 0.997 (0.001)
		& \multicolumn{1}{l} {0.997 (0.002)} 
		& \multicolumn{1}{l} {0.994 (0.002)} \\ 
		\multicolumn{1}{l}{DTLZ2}  
		& \multicolumn{1}{l}{0.923 (0.002)} 
		& \multicolumn{1}{l}{\textbf{0.924 (0.002)}} 
		& \multicolumn{1}{l}{0.921 (0.002)} 
		& 0.920 (0.003)
		& \multicolumn{1}{l} {0.915 (0.003)} 
		& \multicolumn{1}{l} {0.912 (0.005)} \\ 
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ3}  
		& \multicolumn{1}{l}{\textbf{0.985 (0.014)}} 
		& \multicolumn{1}{l}{0.982 (0.016)} 
		& \multicolumn{1}{l}{0.985 (0.018)} 
		& 0.976 (0.017)
		& \multicolumn{1}{l} {0.974 (0.019)} 
		& \multicolumn{1}{l} {0.948 (0.021)} \\ 
		\multicolumn{1}{l}{DTLZ4}  
		& \multicolumn{1}{l}{\textbf{0.977 (0.001)}} 
		& \multicolumn{1}{l}{\textbf{0.977 (0.001)}} 
		& \multicolumn{1}{l}{0.975 (0.001)} 
		& 0.974 (0.002)
		& \multicolumn{1}{l} {0.972 (0.002)} 
		& \multicolumn{1}{l} {0.971 (0.002)} \\ 
	    \rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ5}  
		& \multicolumn{1}{l}{0.923 (0.002)} 
		& \multicolumn{1}{l}{\textbf{0.924 (0.002)}} 
		& \multicolumn{1}{l}{0.921 (0.002)} 
		& 0.920 (0.003)
		& \multicolumn{1}{l} {0.915 (0.003)} 
		& \multicolumn{1}{l} {0.912 (0.005)}\\ 
		\multicolumn{1}{l}{DTLZ6}  
		& \multicolumn{1}{l}{\textbf{1.000 (0.001)}} 
		& \multicolumn{1}{l}{0.980 (0.020)} 
		& \multicolumn{1}{l}{0.907 (0.026)} 
		& 0.823 (0.037)
		& \multicolumn{1}{l} {0.765 (0.033)} 
		& \multicolumn{1}{l} {0.688 (0.049)}  \\ 
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ7}  
		& \multicolumn{1}{l}{\textbf{0.885 (0.027)}} 
		& \multicolumn{1}{l}{0.809 (0.035)} 
		& \multicolumn{1}{l}{0.696 (0.028)} 
		& 0.642 (0.043)
		& \multicolumn{1}{l} {0.595 (0.040)} 
		& \multicolumn{1}{l} {0.552 (0.028)} \\ 
		\cline{6-6}
		\hline
			\end{tabular}
		\end{table*}

==> files/igd_medians.tex <==
% [FELIPE] I'll probably modify these tables, possibly to inform means and standard errors. I'll also highlight a few other aspects in the caption (such as the number of repeated runs, $n = 21$.)
\begin{table*}[!t]
	\centering
	\normalsize
	\caption[IGD medians and standard deviations.]{IGD medians and standard deviations (in parenthesis) for every problem and technique. The best point value for each problem is indicated in boldface.}
	\label{table_igd_threshold}
	\begin{tabular}{lllllll}
	\hline
		\rowcolor[gray]{.7} \multicolumn{1}{|l|}{\textbf{IGD}}         & \multicolumn{1}{l|}{10\%} & \multicolumn{1}{l|}{20\%} & \multicolumn{1}{l|}{40\%} & \multicolumn{1}{l|}{60\%} & \multicolumn{1}{l|}{80\%} & \multicolumn{1}{l|}{100\%}\\ \hline \hline  \hline
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF1}              & \multicolumn{1}{l}{0.271 (0.033)} 
		     & \multicolumn{1}{l}{\textbf{0.261 (0.038)}} 
		     & \multicolumn{1}{l}{0.340 (0.043)} 
		     & 0.425 (0.044)            
		     & \multicolumn{1}{l} {0.474 (0.049)}  
		    & \multicolumn{1}{l} {0.558 (0.056)} \\ 
		
		\multicolumn{1}{l} {UF2}              
		& \multicolumn{1}{l}{0.102 (0.012)} 
		& \multicolumn{1}{l}{0.100 (0.009)}
		& \multicolumn{1}{l}{0.104 (0.009)} 
		& 0.109 (0.008)            
		&\multicolumn{1}{l} {0.114 (0.011)} &\multicolumn{1}{l} {0.122 (0.008)} \\ 
		
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF3}              
		& \multicolumn{1}{l}{\textbf{0.278 (0.011)}} 
		     & \multicolumn{1}{l}{0.280 (0.010)}
		     & \multicolumn{1}{l}{0.289 (0.010)} 
		     & 0.293 (0.011)            
		     & \multicolumn{1}{l} {0.301 (0.008)}  
		     & \multicolumn{1}{l} {0.306 (0.007)}  \\  
		     
		\multicolumn{1}{l} {UF4}              
		& \multicolumn{1}{l}{0.109 (0.003)} 
		& \multicolumn{1}{l}{\textbf{0.108 (0.003)}} 
		& \multicolumn{1}{l}{0.109 (0.002)} 
		& 0.110 (0.003)            
		&\multicolumn{1}{l} {0.111 (0.003)} 
		&\multicolumn{1}{l} {0.112 (0.003)}  \\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF5}              
		& \multicolumn{1}{l}{1.064 (0.094)}
		     & \multicolumn{1}{l}{\textbf{1.060 (0.070)}}
		     & \multicolumn{1}{l}{1.229 (0.063)} 
		     & 1.372 (0.073)            
		     & \multicolumn{1}{l} {1.524 (0.076)}  
		     & \multicolumn{1}{l} {1.723 (0.059)}  \\ 
		     
	     \multicolumn{1}{l} {UF6}              
		& \multicolumn{1}{l}{\textbf{0.283 (0.052)}} 
		& \multicolumn{1}{l}{0.295 (0.048)} 
		& \multicolumn{1}{l}{0.381 (0.053)} 
		& 0.436 (0.045)            
		&\multicolumn{1}{l} {0.503 (0.503)} 
		&\multicolumn{1}{l} {0.579 (0.067)}  \\
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF7}              
		& \multicolumn{1}{l}{\textbf{0.245 (0.044)}}
		     & \multicolumn{1}{l}{0.284 (0.041)}
		     & \multicolumn{1}{l}{0.342 (0.053)} 
		     & 0.411 (0.065)            
		     & \multicolumn{1}{l} {0.452 (0.067)}  
		     & \multicolumn{1}{l} {0.529 (0.054)}  \\ 
		     
		\multicolumn{1}{l} {UF8}              
		& \multicolumn{1}{l}{0.270 (0.026)} 
		& \multicolumn{1}{l}{0.256 (0.017)}
		& \multicolumn{1}{l}{\textbf{0.254 (0.021)}} 
		& 0.267 (0.016)            
		&\multicolumn{1}{l} {0.275 (0.017)} 
		&\multicolumn{1}{l} {0.316 (0.025)} \\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{UF9}             
		& \multicolumn{1}{l}{\textbf{0.419 (0.020)}}
		     & \multicolumn{1}{l}{0.425 (0.024)}
		     & \multicolumn{1}{l}{0.444 (0.019)} 
		     & 0.445 (0.021)            
		     & \multicolumn{1}{l} {0.460 (0.022)}  
		     & \multicolumn{1}{l} {0.470 (0.018)} \\ 
		     
		     \multicolumn{1}{l}{UF10}              
		     & \multicolumn{1}{l}{\textbf{1.986 (0.485)}} 
		    & \multicolumn{1}{l}{2.294 (0.306)} 
		    & \multicolumn{1}{l}{2.708 (0.179)} 
    		& 2.875 (0.206)             
    		&\multicolumn{1}{l} {3.210 (0.194)} 
    		&\multicolumn{1}{l} {3.379 (0.164)}   \\ 
		\hline \hline \hline
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ1}                  
		& \multicolumn{1}{l}{\textbf{189.9 (115.0)}} 
		& \multicolumn{1}{l}{192.2 (138.2)} 
		& \multicolumn{1}{l}{235.6 (117.2)} 
		& 251.1 (117.5)      
		& \multicolumn{1}{l} {307.1 (144.6)} 
		& \multicolumn{1}{l} {436.0 (131.7)} \\
		
		\multicolumn{1}{l}{DTLZ2}     
		& \multicolumn{1}{l}{0.115 (0.015)} 
		& \multicolumn{1}{l}{\textbf{0.110 (0.014)}} 
		& \multicolumn{1}{l}{0.129 (0.016)}
		& 0.141 (0.021)     
		& \multicolumn{1}{l} {0.156 (0.017)} 
		& \multicolumn{1}{l} {0.186 (0.025)}  \\
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ3}
		& \multicolumn{1}{l}{660.2 (338.2)} 
		& \multicolumn{1}{l}{716.3 (403.8)} 
		& \multicolumn{1}{l}{\textbf{625.9 (401.8)}} 
		& 843.4 (389.3)      
		& \multicolumn{1}{l} {814.5 (378.9)}
		& \multicolumn{1}{l} {1075 (402.1)} \\ 
		
		\multicolumn{1}{l}{DTLZ4}     
		& \multicolumn{1}{l}{\textbf{0.105 (0.04)}} 
		& \multicolumn{1}{l}{0.108 (0.023)} 
		& \multicolumn{1}{l}{0.135 (0.029)}
		& 0.169 (0.056)     
		& \multicolumn{1}{l} {0.207 (0.065)} 
		& \multicolumn{1}{l} {0.234 (0.039)}  \\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ5}
		& \multicolumn{1}{l}{0.111 (0.016)} 
		& \multicolumn{1}{l}{\textbf{0.107 (0.014)}} 
		& \multicolumn{1}{l}{0.130 (0.016)} 
		& 0.136 (0.022)      
		& \multicolumn{1}{l} {0.165 (0.017)}
		& \multicolumn{1}{l} {0.187 (0.027)}  \\ 
		
		\multicolumn{1}{l}{DTLZ6}     
		& \multicolumn{1}{l}{\textbf{0.009 (0.623)}} 
		& \multicolumn{1}{l}{5.367 (2.913)} 
		& \multicolumn{1}{l}{12.24 (2.039)}
		& 17.26 (2.215)     
		& \multicolumn{1}{l} {20.81 (2.037)} 
		& \multicolumn{1}{l} {23.67 (2.300)}  \\ 
		
		\rowcolor[gray]{.95}\multicolumn{1}{l}{DTLZ7}
		& \multicolumn{1}{l}{\textbf{0.326 (0.263)}} 
		& \multicolumn{1}{l}{1.047 (0.432)}
		& \multicolumn{1}{l}{2.394 (0.378)} 
		& 3.161 (0.557)      
		& \multicolumn{1}{l} {3.488 (0.409)}
		& \multicolumn{1}{l} {3.923 (0.266)} \\ 
		\cline{6-6}
		\hline
			\end{tabular}
		\end{table*}
		%

==> files/stats_HV.tex <==
\begin{table*}[htbp]
	\begin{center}
	\normalsize
		\caption{Statistical analysis of the HV difference between each different setting values on the Partial Update Strategy, paired on the benchmark functions, using the Pairwise Wilcoxon Rank Sum test. ``$\leftarrow$" indicates superiority of the row method, while ``$\uparrow$" indicates superiority of the column method. ``$\simeq$" 
			indicates no statistical difference.}
		\label{chap4:statistics_fix_hv}
		\begin{tabular}{llllllll}
			\hline
			\rowcolor[gray]{.7} \multicolumn{1}{|l|}{}         & \multicolumn{1}{l|}{10\%} & \multicolumn{1}{l|}{20\%} & \multicolumn{1}{l|}{40\%} & \multicolumn{1}{l|}{60\%} & \multicolumn{1}{l|}{80\%} & \multicolumn{1}{l|}{100\%} \\ \hline \hline  \hline
			
			10\% & - & 0.21178 $\simeq$ &  0.00012 $\leftarrow$ & 1.8e-08 $\leftarrow$ & 2.6e-12 $\leftarrow$ &  4.7e-16 $\leftarrow$ \\
			
			\rowcolor[gray]{.95} 20\% & 0.21178 $\simeq$  & -  & 0.00254 $\leftarrow$  & 1.0e-06 $\leftarrow$ & 1.3e-10 $\leftarrow$ & 1.0e-14 $\leftarrow$  \\
			
			40\% & 0.00012 $\uparrow$ & 0.00254 $\uparrow$ & - & 0.12248 $\simeq$ & 0.00084  $\leftarrow$ &  3.0e-07 $\leftarrow$\\			
			
			\rowcolor[gray]{.95} 60\% & 1.8e-08 $\uparrow$  & 1.0e-06 $\uparrow$   & 0.12248 $\simeq$  & - & 0.09186 $\simeq$ & 0.00020 $\leftarrow$  \\
			
			80\% & 2.6e-12 $\uparrow$ & 1.3e-10 $\uparrow$ & 0.00084 $\uparrow$ & 0.09186 $\simeq$ & - &  0.06252 \\
			
			\rowcolor[gray]{.95} 100\% & 4.7e-16 $\uparrow$  & 1.0e-14 $\uparrow$   & 3.0e-07 $\uparrow$  & 0.00020 $\uparrow$ & 0.06252 $\simeq$ & -  \\
            \hline
		\end{tabular}
	\end{center}
\end{table*}
